GeoResponder: Towards Building Geospatial LLMs for Time-Critical Disaster Response

LLMs excel at linguistic tasks but lack the inner geospatial capabilities needed for time-critical disaster response, where reasoning about road networks, coordinates, and access to essential infrastructure such as hospitals, shelters, and pharmacies is vital. We introduce GeoResponder, a framework that instills robust spatial reasoning through a scaffolded instruction-tuning curriculum. By stratifying geospatial learning into different cognitive layers, we anchor semantic knowledge to the continuous coordinate manifold and enforce the internalization of spatial axioms. Extensive evaluations across four topologically distinct cities and diverse tasks demonstrate that GeoResponder significantly outperforms both state-of-the-art foundation models and domain-specific baselines. These results suggest that LLMs can begin to internalize and generalize geospatial structures, pointing toward the future development of language models capable of supporting disaster response needs.

==> baselines.tex <==

% section discussing baselines and prompt engineering techniques used

% ------------- scratch
% In this section we will introduce the baselines that we will be using to compare models trained with RoadMind framework against. we will use the instruct fine tuned open source models qwen, llama and mistral (same versions as mentioned before). we also use 4o mini (only with the prompt engineering techniques and cheat sheets for cost purposes). we will also provide these baselines with strong prompting techniques such as chain of thought, few shot. We will even go further and provide these models with "cheat sheets" which are contextual grounding and QSF learning. QSF learning, as introduced by \cite{AEF:25} refers to smartly curated few shot examples, that are relevant to the prompt that is being answered. in \cite{AEF:25} the few shot examples were chosen from a database based on semantic similarity to the prompt (the top most similar examples to the prompt were used). in this case, we will use distance as the similarity metric. qsf will only be used for the road retrieal tasks and works this way. we retrieve 1000 random sample points from the AOI and find their actual nearest roads, and directional nearest roads. when we want to run models on a new test point p, we calculate the distance from p to all of the 1000 points in our db, and then get the top 10 closest, and use them as few shot examples. the idea here is that points that are close together have a higher chance of sharing the same nearest roads. this only applies for the road retrieval tasks. for the other tasks we still use all the other techniques but not qsf. contextual grounding is giving the model some relevant in context information similar to what is done in \cite{manvi:24}. in the case of the road retrieval tasks, the context given is all the road names within 4 km of the point. in the case of the road metadata prediction tasks, for segment length, the context is simply the range of segment lengths in aoi. maxspeed is the list of possible maxspeeds. the lanes is list of possible lanes. road name is also list of road names in 4 km (same as before). for spatial calculation tasks context and qsf don't apply, so we use cot and few shot as the enhancement techniques. 


% ------------------- cleaned up version
\subsection{Baselines and Prompting Enhancements}
\label{sec:baselines}

% To evaluate the effectiveness of the \textsc{RoadMind} framework, we compare against several strong open-source instruction-tuned language models: \textbf{Qwen 3 8B}, \textbf{LLaMA 3.1 8B}, and \textbf{Mistral 7B v0.3}, using the same versions as described earlier. Additionally, we include \textbf{GPT-4o Mini}, which is evaluated only with prompting-based techniques (not fine-tuning), due to cost constraints.

% % All baselines are evaluated using advanced prompting strategies, including:
% % \begin{itemize}
% %     \item \textbf{Chain-of-Thought (CoT)} reasoning;
% %     \item \textbf{Few-shot learning};
% %     \item \textbf{Contextual Grounding}, where the prompt includes structured, task-relevant information from OSM similar to  \cite{manvi:24};
% %     \item \textbf{Query-Specific Few-shot (QSF) Learning}~\cite{AEF:25}, a retrieval-based approach to selecting semantically relevant few-shot examples.
% % \end{itemize}

% All baselines are evaluated using advanced prompting strategies, which we will call as "cheat sheets". These strategies include \textbf{Chain-of-Thought (CoT)} reasoning, \textbf{Few-shot learning}, \textbf{Contextual Grounding} -where the prompt includes structured, task-relevant information from OSM similar to  \cite{manvi:24}-, and \textbf{Query-Specific Few-shot (QSF) Learning}~\cite{AEF:25}, a retrieval-based approach to selecting semantically relevant few-shot examples.

% \textbf{QSF Learning} is applied only to the road retrieval tasks. Inspired by~\cite{AEF:25}, we construct a database of 1,000 randomly sampled points from the area of interest (AOI), each annotated with their nearest road and directional nearest roads. For a new test point $p$, we compute its distance to all stored points and retrieve the 10 closest examples to use as few-shot demonstrations. This exploits the locality property: nearby points are likely to share similar nearest roads.

% \textbf{Contextual Grounding} is used in all tasks except the spatial reasoning ones. The contextual inputs vary by task:
% \begin{itemize}
%     \item \textit{Road retrieval tasks:} a list of road names within a 4km radius of the query point;
%     \item \textit{Segment metadata prediction:}
%     \begin{itemize}
%         \item Length: range of segment lengths in the AOI;
%         \item Maxspeed: list of possible maxspeed values;
%         \item Lanes: list of possible lane counts;
%         \item Road name: same 4km-local road name list as above.
%     \end{itemize}
%     \item \textit{Distance and direction tasks:} Contextual and QSF enhancements are not applicable; only CoT and few-shot prompting are used.
% \end{itemize}




To evaluate \textsc{RoadMind}, we compare against strong open-source instruction-tuned models: Qwen 3 8B, LLaMA 3.1 8B, and Mistral 7B v0.3, as well as GPT-4o Mini, which is used only with prompting due to cost constraints.

We use two prompting settings for the open-source models: \textbf{direct prompting} (simple, task-specific queries without enhancements) and \textbf{cheat-sheet prompting}, which combines several advanced strategies:
\textbf{Chain-of-Thought (CoT)} reasoning, \textbf{few-shot learning}, \textbf{contextual grounding} (injecting structured OSM information, as in \cite{manvi:24}), and \textbf{Query-Specific Few-shot (QSF)} learning \cite{AEF:25}, which retrieves semantically similar few-shot examples.

\textbf{QSF} is applied only to road retrieval tasks. Following \cite{AEF:25}, we build a database of 1,000 sampled points in the area of interest (AOI), each annotated with nearest and directional roads. For a new test point $p$, we retrieve its 10 closest examples using haversine distance and use them as few-shot demonstrations, leveraging spatial locality.


\textbf{Contextual grounding} is applied to all tasks except spatial reasoning. For road retrieval, the prompt includes road names within a 4km radius of the query point. For metadata prediction, we provide distributional hints such as typical \texttt{maxspeed} values, lane counts, segment lengths, and nearby road names. For distance and direction estimation, neither contextual grounding nor QSF is applicable; only Chain-of-Thought and few-shot prompting are used.

